FL-NTK: A Neural Tangent Kernel-based Framework for Federated Learning Convergence Analysis

Federated Learning (FL) is an emerging learning scheme that allows different distributed clients to train deep neural networks together without data sharing. Neural networks have become popular due to their unprecedented success. To the best of our knowledge, the theoretical guarantees of FL concerning neural networks with explicit forms and multi-step updates are unexplored. Nevertheless, training analysis of neural networks in FL is non-trivial for two reasons: first, the objective loss function we are optimizing is non-smooth and non-convex, and second, we are even not updating in the gradient direction. Existing convergence results for gradient descent-based methods heavily rely on the fact that the gradient direction is used for updating. This paper presents a new class of convergence analysis for FL, Federated Learning Neural Tangent Kernel (FL-NTK), which corresponds to overparamterized ReLU neural networks trained by gradient descent in FL and is inspired by the analysis in Neural Tangent Kernel (NTK). Theoretically, FL-NTK converges to a global-optimal solution at a linear rate with properly tuned learning parameters. Furthermore, with proper distributional assumptions, FL-NTK can also achieve good generalization.

==> gen.tex <==
%!TEX root=main.tex
\section{Training Speed}\label{sec:training_speed}


\Zhao{I can't remember our plan. Should I read this?}\Baihe{This section is from \cite{sy19}.} \Zhao{I knew it is from \cite{sy19}, since I copied it. My question is : are we going to modify the proof to federated learning setting?}
\Xin{We should remove this section.}
In this section we change the initialization scheme as initialize each $w_r(0)$ as ${\N}(0,\kappa^2 I)$.
It is not hard to see that this just introduce an extra $\kappa^{-2}$ term for every occurrence of $m$.
\begin{algorithm} % enter the algorithm environment
\caption{Training neural network using gradient descent with small variance.}
\label{alg:variance} 
\begin{algorithmic}[1]
    \Procedure{NNTraining}{$\{(x_i,y_i)\}_{i\in [n]}$}
    \State $w_r(0) \sim \N(0,\kappa^2I_d)$ for $r\in [m]$.
    % \State $u(1) \leftarrow 0$
    \For{$t=1 \to T$}
        \State $u(t) \leftarrow \frac{1}{ \sqrt{m} } \sum_{r=1}^m a_r \sigma(w_r(t)^\top X) $ \Comment{$u(t) = f(W(t),x,a) \in \R^n$, it takes $O(mnd)$ time}
        \For{$r = 1 \to m$}
            \For{$i = 1 \to n$} 
                \State $Q_{i,:} \leftarrow \frac{1}{\sqrt{m}}a_r\sigma'(w_r(t)^\top x_i)x_i^\top$ \Comment{$Q_{i,:} = \frac{\partial f(W(t),x_i,a)}{\partial w_r}$, it takes $O(d)$ time}
            \EndFor
            \State $\text{grad}_r \leftarrow - Q^\top (y - u(t) ) $%$+\lambda w_r(t)$ 
            \Comment{ $Q = \frac{\partial f} {\partial w_r } \in \R^{n \times d}$, it takes $O(nd)$ time }
            \State $w_r(t+1) \leftarrow w_r(t) - \eta \cdot \text{grad}_r $
        \EndFor
    \EndFor
    \State \Return $W$
    \EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{lemma}[Restatement of Lemma \ref{lem:4.1}, improved Version of Lemma C.1 in \cite{adhlw19}]\label{lem:4.1_restatement}
Recall that $\lambda=\lambda_{\min}(H^{\cts})>0$.
Fix $\kappa>0$.
Let $m = \Omega( \lambda^{-4} \kappa^{-2} n^4 \log (n/\delta) )$, we i.i.d. initialize $w_r \in {\N}(0,\kappa^2 I)$, $a_r$ sampled from $\{-1,+1\}$ uniformly at random for $r\in [m]$, and we set the step size $\eta = O( \lambda / n^2 )$ then with probability at least $1-\delta$ over the random initialization we have for $k = 0,1,2,\cdots$.
\begin{align*}
\| w_r(k+1) - w_r(0) \|_2 \leq \frac{ 4 \sqrt{n} \| y - u (0) \|_2 }{ \sqrt{m} \lambda }.
\end{align*}
\end{lemma}


% \begin{lemma}[Improved version of Lemma C.2 in \cite{adhlw19}]\label{lem:HZ_norm_bound}
% For integer $k\geq 0$,
% define $Z(k)\in \mathbb{R}^{md\times n}$ as the matrix
% \begin{align*}
% Z(k)=\frac{1}{\sqrt{m}} \begin{pmatrix} a_1x_1 {\bf 1}_{ w_1(k)^\top x_1 \geq 0} & \cdots & a_1x_n {\bf 1}_{ w_1(k)^\top x_n \geq 0}\\
% \vdots & \ddots & \vdots\\
% a_mx_1 {\bf 1}_{ w_m(k)^\top x_1 \geq 0} & \cdots & a_mx_n {\bf 1}_{ w_m(k)^\top x_n \geq 0}\\
% \end{pmatrix}.
% \end{align*}
% Under the same setting as Lemma \ref{lem:4.1_restatement},
% with probability at least $1-2\delta$ over the random initialization, for $k = 0,1,2,\cdots$ we have
% \begin{align*}
% \|H(k)-H(0)\|_F&= O \Big(  n^2\sqrt{\log(m/\delta)\log^2(n/\delta)}  /  ( \kappa\lambda\sqrt{m} ) \Big) , \\
% \|Z(k)-Z(0)\|_F&=O() .
% \end{align*}
% \end{lemma}
% \begin{proof}
% This proof is analogous to the proof of Lemma \ref{lem:3.2}.
% Let 
% \begin{align*}
% R=\frac{ C n\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \sqrt{m} \lambda }
% \end{align*}
% for some universal constant $C>0$.
% Let $E$ be the event that $\|w_r(k)-w_r(0)\|_2\leq R$ for all $k\geq 0$ and $r\in [m]$.

% By Claim \ref{cla:yu0},
% plugging 
% \begin{align*}
% \| y - u ( 0 ) \|_2 = O ( \sqrt{ n \log(m/\delta)\log^2(n/\delta) } )
% \end{align*}
% into Lemma \ref{lem:4.1_restatement},
% we have event $E$ happens with probability at least $1-\delta$,
% In the following proof we just assume event $E$ happens.

% We start with bounding $\|H(k)-H(0)\|_F$ as 
% \begin{align*}
% \|H(k)-H(0)\|_F^2= & ~ \sum_{i=1}^n \sum_{j=1}^n | H(k)_{i,j} - H(0)_{i,j} |^2 \\
% %= & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ w_r(0)^\top x_i \geq 0, w_r(0)^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right|^2 \\
% \leq & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n \left( \sum_{r=1}^m {\bf 1}_{ w_r(k)^\top x_i \geq 0, w_r(k)^\top x_j \geq 0} - {\bf 1}_{ w_r(0)^\top x_i \geq 0 , w_r(0)^\top x_j \geq 0 } \right)^2 \\
% = & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n  \Big( \sum_{r=1}^m s_{r,i,j} \Big)^2 ,
% \end{align*}

% where the last step follows from for each $r,i,j$, we define
% \begin{align*}
% s_{r,i,j} :=  {\bf 1}_{ w_r(k)^\top x_i \geq 0, w_r(k)^\top x_j \geq 0} - {\bf 1}_{ w_r(0)^\top x_i \geq 0 , w_r(0)^\top x_j \geq 0 } .
% \end{align*} 

% We consider $i,j$ to be fixed. We simplify $s_{r,i,j}$ to $s_r$.
% Then $s_r$ is a random variable that only depends on $w_r(0)$.
% Since $\{w_r(0)\}_{r=1}^m$ are independent,
% $\{s_r\}_{r=1}^m$ are also mutually independent.


% We define the event
% \begin{align*}
% A_{i,r} = \left\{ \exists u : \| u - w_r(0) \|_2 \leq R, {\bf 1}_{ x_i^\top w_r(0) \geq 0 } \neq {\bf 1}_{ x_i^\top u \geq 0 } \right\}.
% \end{align*}
% Note this event happens if and only if $| w_r(0)^\top x_i | < R$. Recall that $w_r(0) \sim \N(0,\kappa^2 I)$. By anti-concentration inequality of Gaussian (Lemma~\ref{lem:anti_gaussian}), we have
% \begin{align}\label{eq:Air_bound}
% \Pr[ A_{i,r} ] = \Pr_{ z \sim \N(0,\kappa^2) } [ | z | < R ] \leq \frac{ 2 R }{ \sqrt{2\pi}\kappa }.
% \end{align}

% Assume $ \|w_r(0)- w_r(k)\|_2\leq R$.
% If   $\neg A_{i,r}$ and $\neg A_{j,r}$ happen,
% then 
% \begin{align*}
% \left| {\bf 1}_{  w_r(k)^\top x_i \geq 0,  w_r(k)^\top x_j \geq 0} - {\bf 1}_{  w_r(0)^\top x_i \geq 0 ,  w_r(0)^\top x_j \geq 0 } \right|=0.
% \end{align*}
% If   $A_{i,r}$ or $A_{j,r}$ happen,
% then 
% \begin{align*}
% \left| {\bf 1}_{  w_r(k)^\top x_i \geq 0,  w_r(k)^\top x_j \geq 0} - {\bf 1}_{  w_r(0)^\top x_i \geq 0 ,  w_r(0)^\top x_j \geq 0 } \right|\leq 1.
% \end{align*}

% So we have 
% \begin{align*}
%  \E_{w_r(0)}[s_r]\leq & ~\E_{w_r(0)} \left[ {\bf 1}_{A_{i,r}\vee A_{j,r}} \right]\\
%  \leq & ~ \Pr[A_{i,r}]+\Pr[A_{j,r}]\\
%  \leq & ~ \frac {4 R\kappa^{-1}}{\sqrt{2\pi}} \\
%  \leq & ~ 2 R\kappa^{-1} ,
% \end{align*}
% and
% \begin{align*}
%     \E_{w_r(0)} \left[ \left(s_r-\E_{w_r(0)}[s_r] \right)^2 \right]
%     = & ~ \E_{w_r(0)}[s_r^2]-\E_{w_r(0)}[s_r]^2 \\
%     \leq & ~ \E_{w_r(0)}[s_r^2] \\
%     \leq & ~ \E_{w_r(0)} \left[ \left( {\bf 1}_{A_{i,r}\vee A_{j,r}} \right)^2 \right] \\
%     \leq & ~ \frac {4R\kappa^{-1}}{\sqrt{2\pi}} \\
%     \leq & ~ 2 R\kappa^{-1} .
% \end{align*}
% We also have $|s_r|\leq 1$.
% So we can apply Bernstein inequality (Lemma~\ref{lem:bernstein}) to get for all $t>0$,{\small
% \begin{align*}
%     \Pr \left[\sum_{r=1}^m s_r\geq 2m R\kappa^{-1} +mt \right]
%     \leq & ~ \Pr \left[\sum_{r=1}^m (s_r-\E[s_r])\geq mt \right]\\
%     \leq & ~ \exp \left( - \frac{ m^2t^2/2 }{ 2m R\kappa^{-1}  + mt/3 } \right).
% \end{align*}}
% Choosing $t = R\kappa^{-1}$, we get
% \begin{align*}
%     \Pr \left[\sum_{r=1}^m s_r\geq 3mR\kappa^{-1} \right]
%     \leq & ~ \exp \left( -\frac{ m^2  (R\kappa^{-1})^2 /2 }{ 2 m  R\kappa^{-1}   +m  R\kappa^{-1} /3 } \right) \\
%      \leq & ~ \exp \left( - m R\kappa^{-1} / 10 \right) .
% \end{align*}
% Thus, we can have
% \begin{align*}
% \Pr \left[ \frac{1}{m} \sum_{r=1}^m s_r \geq 3  R\kappa^{-1} \right] \leq \exp( - m R\kappa^{-1} /10 ).
% \end{align*}
% Therefore, by applying union bound all $(i,j)\in [n]\times [n]$, we have
% with probability at least $1-n^2\exp( - m R\kappa^{-1} /10 )$,
% \begin{align*}
% \|H(k)-H(0)\|_F^2\leq n^2(3  R\kappa^{-1})^2.
% \end{align*}
% With the choice of $m=\Omega( \lambda^{-4} \kappa^{-2} n^4 \log (n/\delta) )$,
% we have $n^2\exp( - m (R\kappa^{-1}+\delta) /10 )\leq \delta$.
% Hence by union bound on the event $E$,
% with probability at least $1-2\delta$,
% \begin{align*}
% \|H(k)-H(0)\|_F =O\left(\frac{ n^2\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m}  }\right).
% \end{align*}


\begin{lemma}[Improved version of Lemma C.2 in \cite{adhlw19}]\label{lem:HZ_norm_bound}
For integer $k\geq 0$,
define $Z(k)\in \mathbb{R}^{md\times n}$ as the matrix
\begin{align*}
Z(k)=\frac{1}{\sqrt{m}} \begin{pmatrix} a_1x_1 {\bf 1}_{ w_1(k)^\top x_1 \geq 0} & \cdots & a_1x_n {\bf 1}_{ w_1(k)^\top x_n \geq 0}\\
\vdots & \ddots & \vdots\\
a_mx_1 {\bf 1}_{ w_m(k)^\top x_1 \geq 0} & \cdots & a_mx_n {\bf 1}_{ w_m(k)^\top x_n \geq 0}\\
\end{pmatrix}.
\end{align*}
Under the same setting as Lemma \ref{lem:4.1_restatement},
with probability at least $1-4\delta$ over the random initialization, for $k = 0,1,2,\cdots$ we have
\begin{align*}
\|H(k)-H(0)\|_F = & ~ O(1) \cdot n \cdot \left( \delta+\frac{ n\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m}  } \right) ,\\
\|Z(k)-Z(0)\|_F = & ~ O(1) \cdot  \left( n \cdot \Big(\delta+\frac{  n\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m} } \Big) \right)^{1/2} .\\
\end{align*}
%\Zhao{Can you check the above equation, originally bracket doesn't match}
\end{lemma}
\begin{remark}
$H(0)$ is just $H^{\dis}$ defined in Lemma \ref{lem:3.1}.
\end{remark}

\begin{proof}
This proof is analogous to the proof of Lemma \ref{lem:3.2}.
Let 
\begin{align*}
R=\frac{ C n\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \sqrt{m} \lambda }
\end{align*}
for some sufficiently small constant $C>0$. %\Zhao{Sufficiently large or sufficiently small?}


By Claim \ref{cla:yu0},
plugging 
\begin{align*}
\|y-u(0)\|_2 = O \Big( \sqrt{ n \log(m/\delta) \log^2(n/\delta) } \Big)
\end{align*}
into Lemma \ref{lem:4.1_restatement},
we have with probability at least $1-\delta$,
$\|w_r(k)-w_r(0)\|_2\leq R$ for all $k\geq 0$ and $r\in [m]$.

We start with bounding $\|H(k)-H(0)\|_F$ as 
\begin{align*}
\|H(k)-H(0)\|_F^2= & ~ \sum_{i=1}^n \sum_{j=1}^n | H(k)_{i,j} - H(0)_{i,j} |^2 \\
%= & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ w_r(0)^\top x_i \geq 0, w_r(0)^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right|^2 \\
\leq & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n \left( \sum_{r=1}^m {\bf 1}_{ w_r(k)^\top x_i \geq 0, w_r(k)^\top x_j \geq 0} - {\bf 1}_{ w_r(0)^\top x_i \geq 0 , w_r(0)^\top x_j \geq 0 } \right)^2 \\
= & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n  \Big( \sum_{r=1}^m s_{r,i,j} \Big)^2 ,
\end{align*}

where the last step follows from for each $r,i,j$, we define
\begin{align*}
s_{r,i,j} :=  {\bf 1}_{ w_r(k)^\top x_i \geq 0, w_r(k)^\top x_j \geq 0} - {\bf 1}_{ w_r(0)^\top x_i \geq 0 , w_r(0)^\top x_j \geq 0 } .
\end{align*} 

We consider $i,j$ to be fixed. We simplify $s_{r,i,j}$ to $s_r$.
Then $s_r$ is a random variable that only depends on $w_r(0)$.
Since $\{w_r(0)\}_{r=1}^m$ are independent,
$\{s_r\}_{r=1}^m$ are also mutually independent.


We define the event
\begin{align*}
A_{i,r} = \left\{ \exists u : \| u - w_r(0) \|_2 \leq R, {\bf 1}_{ x_i^\top w_r(0) \geq 0 } \neq {\bf 1}_{ x_i^\top u \geq 0 } \right\}.
\end{align*}
Note this event happens if and only if $| w_r(0)^\top x_i | < R$. Recall that $w_r(0) \sim \N(0,\kappa^2 I)$. By anti-concentration inequality of Gaussian (Lemma~\ref{lem:anti_gaussian}), we have
\begin{align}\label{eq:Air_bound_variance}
\Pr[ A_{i,r} ] = \Pr_{ z \sim \N(0,\kappa^2) } [ | z | < R ] \leq \frac{ 2 R }{ \sqrt{2\pi}\kappa }.
\end{align}

Assume $ \|w_r(0)- w_r(k)\|_2\leq R$.
If   $\neg A_{i,r}$ and $\neg A_{j,r}$ happen,
then 
\begin{align*}
\left| {\bf 1}_{  w_r(k)^\top x_i \geq 0,  w_r(k)^\top x_j \geq 0} - {\bf 1}_{  w_r(0)^\top x_i \geq 0 ,  w_r(0)^\top x_j \geq 0 } \right|=0.
\end{align*}
If   $A_{i,r}$ or $A_{j,r}$ happen,
then 
\begin{align*}
\left| {\bf 1}_{  w_r(k)^\top x_i \geq 0,  w_r(k)^\top x_j \geq 0} - {\bf 1}_{  w_r(0)^\top x_i \geq 0 ,  w_r(0)^\top x_j \geq 0 } \right|\leq 1.
\end{align*}
Finally, if $\|w_r(0)- w_r(k)\|_2> R$, we still have
\begin{align*}
\left| {\bf 1}_{  w_r(k)^\top x_i \geq 0,  w_r(k)^\top x_j \geq 0} - {\bf 1}_{  w_r(0)^\top x_i \geq 0 ,  w_r(0)^\top x_j \geq 0 } \right|\leq 1.
\end{align*}
So we have 
\begin{align*}
 \E_{w_r(0)}[s_r]\leq & ~\E_{w_r(0)} \left[ {\bf 1}_{A_{i,r}\vee A_{j,r}} \right] +  \Pr[\|w_r(0)- w_r(k)\|_2> R]\\
 \leq & ~ \Pr[A_{i,r}]+\Pr[A_{j,r}] +  \Pr[\|w_r(0)- w_r(k)\|_2> R]\\
 \leq & ~ \frac {4 R\kappa^{-1}}{\sqrt{2\pi}}+\delta \\
 \leq & ~ 2 R\kappa^{-1}+\delta ,
\end{align*}
and
\begin{align*}
    \E_{w_r(0)} \left[ \left(s_r-\E_{w_r(0)}[s_r] \right)^2 \right]
    = & ~ \E_{w_r(0)}[s_r^2]-\E_{w_r(0)}[s_r]^2 \\
    \leq & ~ \E_{w_r(0)}[s_r^2]\\
    \leq & ~\E_{w_r(0)} \left[ \left( {\bf 1}_{A_{i,r}\vee A_{j,r}} \right)^2 \right]+\delta \\
     \leq & ~ \frac {4R\kappa^{-1}}{\sqrt{2\pi}}+\delta \\
     \leq & ~ 2 R\kappa^{-1} + \delta .
\end{align*}
We also have $|s_r|\leq 1$.
So we can apply Bernstein inequality (Lemma~\ref{lem:bernstein}) to get for all $t>0$,
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 2m R\kappa^{-1}+ m \delta +mt \right]
    \leq & ~ \Pr \left[\sum_{r=1}^m (s_r-\E[s_r])\geq mt \right]\\
    \leq & ~ \exp \left( - \frac{ m^2t^2/2 }{ 2m R\kappa^{-1} +m \delta   + mt/3 } \right).
\end{align*}
Choosing $t = R\kappa^{-1}+2\delta$, we get
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 3m(R\kappa^{-1}+\delta)  \right]
    \leq & ~ \exp \left( -\frac{ m^2  (R\kappa^{-1}+\delta)^2 /2 }{ 2 m  R\kappa^{-1}  +m \delta +m  (R\kappa^{-1}+2\delta) /3 } \right) \\
     \leq & ~ \exp \left( - m (R\kappa^{-1}+\delta) / 10 \right) .
\end{align*}
Thus, we can have
\begin{align*}
\Pr \left[ \frac{1}{m} \sum_{r=1}^m s_r \geq 3  R\kappa^{-1}+3\delta \right] \leq \exp( - m (R\kappa^{-1}+\delta) /10 ).
\end{align*}
Therefore, by allying union bound all $(i,j)\in [n]\times [n]$, we have
with probability at least $1-n^2\exp( - m (R\kappa^{-1}+\delta) /10 )$,
\begin{align*}
\|H(k)-H(0)\|_F^2\leq n^2(3  R\kappa^{-1}+3\delta)^2
\end{align*}



Similarly, to bound $\|Z(k)-Z(0)\|_F$,
we have
\begin{align*}
\|Z(k)-Z(0)\|_F^2
%= & ~ \frac{1}{m^2} \sum_{i=1}^n \sum_{j=1}^n \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ w_r(0)^\top x_i \geq 0, w_r(0)^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right|^2 \\
= & ~ \frac{1}{m} \sum_{r=1}^m \sum_{i=1}^n \left( \|x_i\|_2 \cdot  a_i({\bf 1}_{ w_r(k)^\top x_i \geq 0}-{\bf 1}_{ w_r(0)^\top x_i \geq 0})\right)^2 \\
= & ~ \frac{1}{m} \sum_{r=1}^m \sum_{i=1}^n  \Big({\bf 1}_{ w_r(k)^\top x_i \geq 0}-{\bf 1}_{ w_r(0)^\top x_i \geq 0} \Big)^2\\
= & ~ \frac{1}{m} \sum_{r=1}^m \sum_{i=1}^n  {\bf 1}_{{\bf 1}_{ w_r(k)^\top x_i \geq 0}\neq {\bf 1}_{ w_r(0)^\top x_i \geq 0}} \\
= & ~ \frac{1}{m}  \sum_{i=1}^n \sum_{r=1}^m {\bf 1}_{{\bf 1}_{ w_r(k)^\top x_i \geq 0}\neq {\bf 1}_{ w_r(0)^\top x_i \geq 0}}.
\end{align*}

Fix $i\in [n]$ and for $r\in [m]$,
define $t_r= {\bf 1}_{{\bf 1}_{ w_r(k)^\top x_i \geq 0}\neq {\bf 1}_{ w_r(0)^\top x_i \geq 0}}$.
If $A_{i,r}$ does not happen and $\|w_r(0)- w_r(k)\|_2\leq R$, %\Zhao{Can you make sure $\| \|_F$ for Frobenius norm, use $\| \|$ matrix spectral norm, use $\| \|_2$ for entry-wise $\ell_2$ norm. Can you remember this?}
we must have $t_r=0$.
Equivalently,
if $t_r=1$,
then either $A_{i,r}$ happens or $\|w_r(0)- w_r(k)\|_2> R$.
Therefore
\begin{align*}
\E_{w_r(0)}[t_r]\leq \Pr[A_{i,r}]+\Pr[\|w_r(0)- w_r(k)\|_2> R]\leq R\kappa^{-1} + \delta.
\end{align*}
Similarly,
\begin{align*}
\E_{w_r(0)}[(t_r-\E_{w_r(0)}[t_r])^2]
= & ~\E_{w_r(0)}[t_r^2]-\E_{w_r(0)}[t_r]^2\\
\leq & ~\E_{w_r(0)}[t_r^2]\\
= & ~\E_{w_r(0)}[t_r]\\
\leq & ~R\kappa^{-1} + \delta.
\end{align*}
So we can apply Bernstein inequality (Lemma~\ref{lem:bernstein}) to get for all $t>0$,
\begin{align*}
    \Pr \left[\sum_{r=1}^m t_r\geq m R\kappa^{-1}+ m \delta +mt \right]
    \leq & ~ \Pr \left[\sum_{r=1}^m (s_r-\E[s_r])\geq mt \right]\\
    \leq & ~ \exp \left( - \frac{ m^2t^2/2 }{ m R\kappa^{-1} +m \delta   + mt/3 } \right).
\end{align*}
Choosing $t = R\kappa^{-1}+\delta$, we get
\begin{align*}
    \Pr \left[\sum_{r=1}^m t_r\geq 2m(R\kappa^{-1}+\delta)  \right]
    \leq & ~ \exp \left( -\frac{ m^2  (R\kappa^{-1}+\delta)^2 /2 }{  m  R\kappa^{-1}  +m \delta +m  (R\kappa^{-1}+\delta) /3 } \right) \\
     \leq & ~ \exp \left( - m (R\kappa^{-1}+\delta) / 10 \right) .
\end{align*}
By applying union bound over $i\in [n]$,
we have with probability at least $1-n\exp \left( - m (R\kappa^{-1}+\delta) / 10 \right) $,
\begin{align*}
\|Z(k)-Z(0)\|_F^2\leq 2n(R\kappa^{-1}+\delta),
\end{align*}
which is exactly what we need.
% Assume event $E$ happens and fix $i\in [n]$.
% If $\neg A_{i,r}$ happens,
% \begin{align*}
% {\bf 1}_{ w_r(k)^\top x_i \geq 0}-{\bf 1}_{ w_r(0)^\top x_i \geq 0}=0.
% \end{align*}
% Otherwise if $A_{i,r}$ happens,
% then
% \begin{align*}
% \left|{\bf 1}_{ w_r(k)^\top x_i \geq 0}-{\bf 1}_{ w_r(0)^\top x_i \geq 0}\right| \leq 1.
% \end{align*}
\end{proof}


We also need the following parametric version of Lemma \ref{lem:3.1}.
\begin{lemma}\label{lem:3.1_para}
Let $H^{\cts}, H^{\dis} \in \R^{n \times n}$ be defined as in Lemma \ref{lem:3.1}.
Then with probability at least $1-\delta$,
\begin{align*}
\| H^{\dis} - H^{\cts} \|_F =O(n\sqrt{\log(n/\delta)/m}).
\end{align*}
\end{lemma}


The main result in this section is the following theorem.
\begin{theorem}[Improvement of Theorem 4.1 in \cite{adhlw19}]\label{thm:generalization_main}
Recall that $\lambda=\lambda_{\min}(H^{\cts})>0$.
Write the eigen-decomposition of $H^{\cts}$ as $H^{\cts}=\sum_{i=1}^n \lambda_i v_i v_i^\top$ where $v_i\in \mathbb{R}^n$ are the eigenvectors,
and $\lambda_i>0$ are the corresponding eigenvalues.
Let 
\begin{align*}
\kappa = & ~ O( \epsilon / ( \sqrt{2n\log ( 2mn / \delta) }\cdot \log ( 4n / \delta ) ) ) \\
m = & ~ \Omega( \lambda^{-4}\kappa^{-2} n^6 \log (n/\delta) ),
\end{align*}
we i.i.d. initialize $w_r \in {\N}(0,\kappa^2I)$, $a_r$ sampled from $\{-1,+1\}$ uniformly at random for $r\in [m]$, and we set the step size $\eta = O( \lambda / n^2 )$,  then with probability at least $1-\delta$ over the random initialization we have for $k = 0,1,2,\cdots$
\begin{align}
\| u (k) - y \|_2 = \left( \sum_{i=1}^n(1-\eta\lambda_i)^{2k}(v_i^\top y)^2 \right)^{1/2} \pm \epsilon.
\end{align}
\end{theorem}
\begin{proof}
Throughout the proof we assume for all $k=0,1,\cdots$ and all $r\in[m]$,
\begin{align*}
\| w_r(k+1) - w_r(0) \|_2 \leq \frac{ 4 \sqrt{n} \| y - u (0) \|_2 }{ \sqrt{m} \lambda }:=R.
\end{align*}
By Lemma \ref{lem:4.1_restatement},
this holds with probability at least $1-\delta$.

By the update rule of gradient descent,
we have for all $i\in [n]$,
\begin{align}\label{eq:gd_update}
u_i(k+1) - u_i(k)
= & ~ \frac{1}{ \sqrt{m} } \sum_{r=1}^m a_r \cdot \left( \phi( w_r(k+1)^\top x_i ) - \phi(w_r(k)^\top x_i ) \right).
\end{align}
Our target is to relate $u(k+1)-u(k)$ with $u(k)-y$.
Recall that for $i\in [n]$,
the subset $S_i$ is defined as
\begin{align*}
    S_i:=\{r\in [m]:\forall 
    w\in \mathbb{R}^d \text{ s.t. } \|w-w_r(0)\|_2\leq R, 
    \mathbf{1}_{w_r(0)^\top x_i\geq 0}=\mathbf{1}_{w^\top x_i\geq 0}\}.
\end{align*}
Hence we split the summation in \ref{eq:gd_update} by $S_i$,
which is
\begin{align*}
u_i(k+1) - u_i(k)=U_1+U_2
\end{align*}
where 
\begin{align*}
U_1:= & ~\frac{1}{ \sqrt{m} } \sum_{r\in S_i} a_r \cdot \left( \phi( w_r(k+1)^\top x_i ) - \phi(w_r(k)^\top x_i ) \right),\\
U_2:= & ~\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} a_r \cdot \left( \phi( w_r(k+1)^\top x_i ) - \phi(w_r(k)^\top x_i ) \right).
\end{align*}
We start with upper bounding $U_2$ by considering $U_2$ as a perturbation term.
\begin{align*}
|U_2|= & ~|\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} a_r \cdot \left( \phi( w_r(k+1)^\top x_i ) - \phi(w_r(k)^\top x_i ) \right)|\\
\leq & ~\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} \left |w_r(k+1)^\top x_i  - w_r(k)^\top x_i  \right|\\
\leq & ~\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} \left \|w_r(k+1)  - w_r(k) \right\|_2\\
=& ~\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} \left \|\eta \frac{ \partial L(W(k)) }{ \partial w_r(k) }\right\|_2\\
 =& ~\frac{1}{ \sqrt{m} } \sum_{r \in \ov{S}_i} \left \|\eta\frac{1}{ \sqrt{m} } \sum_{j=1}^n ( u_j(k) - y_j ) a_r x_j {\bf 1}_{ w_r(k)^\top x_j \geq 0 }\right\|_2\\
 \leq & ~\frac{\eta}{ m} \sum_{r \in \ov{S}_i} \sum_{j=1}^n\left | u_j(k) - y_j \right|\\
  \leq & ~\frac{\eta\sqrt{n}|\ov{S}_i|}{ m} \left\| u(k) - y \right\|_2\\
\end{align*}
%\Xin{Here can use similar trick to reduce $\sqrt{n}$ to $\alpha$}
where the second step follows from $\phi(\cdot)$ is 1-Lipschitz,
the third step follows from $\|x_i\|_2=1$,
the fifth step follows from Eq. \eqref{eq:gradient},
and the sixth step follows from triangle inequality.


We then bound $U_1$ as follows:
\begin{align*}
& ~ \frac{1}{ \sqrt{m} } \sum_{r\in S_i} a_r \cdot \left( \phi( w_r(k+1)^\top x_i ) - \phi(w_r(k)^\top x_i ) \right)\\
= & ~\frac{1}{ \sqrt{m} } \sum_{r\in S_i} a_r{\bf 1}_{w_r(k)^\top x_i\geq 0} \cdot \left(  w_r(k+1)^\top x_i  - w_r(k)^\top x_i \right)\\
= & ~\frac{1}{ \sqrt{m} } \sum_{r\in S_i} a_r{\bf 1}_{w_r(k)^\top x_i\geq 0} \cdot \left\langle  -\eta\frac{1}{ \sqrt{m} } \sum_{j=1}^n ( u_j(k) - y_j ) a_r x_j {\bf 1}_{ w_r(k)^\top x_j \geq 0 } ,x_i \right\rangle\\
= & ~ - \frac{\eta}{m}\sum_{j=1}^n ( u_j(k) - y_j )x_j^\top x_i \sum_{r\in S_i}{\bf 1}_{w_r(k)^\top x_i\geq 0}{\bf 1}_{w_r(k)^\top x_j\geq 0}\\
= & ~ - \frac{\eta}{m}\sum_{j=1}^n ( u_j(k) - y_j )x_j^\top x_i \sum_{r=1}^{m}{\bf 1}_{w_r(k)^\top x_i\geq 0}{\bf 1}_{w_r(k)^\top x_j\geq 0} \\
 & ~ + \frac{\eta}{m}\sum_{j=1}^n ( u_j(k) - y_j )x_j^\top x_i \sum_{r\in \ov{S}_i}{\bf 1}_{w_r(k)^\top x_i\geq 0}{\bf 1}_{w_r(k)^\top x_j\geq 0}\\
=: & ~-\eta \sum_{j=1}^{n}( u_j(k) - y_j )H_{ij}(k)+\epsilon(k)'
\end{align*}
where the first step follows from the definition of $S_i$,
the fifth step follows from the construction of the matrix $H$.
Moreover,
analogs to upper bounding $U_2$,
we also have
\begin{align*}
|\epsilon(k)'|\leq \frac{\eta\sqrt{n}|\ov{S}_i|}{ m} \left\| u(k) - y \right\|_2.
\end{align*}
Hence by considering all $i\in [n]$,
we have
\begin{align}\label{eq:uk_diff}
u(k+1)-u(k)=-\eta H(k)(u(k)-y)+\epsilon(k)
\end{align}
where $\epsilon(k)\in \mathbb{R}^n$ and the norm of $\epsilon(k)$ can be upper bounded by
\begin{align}\label{eq:eps_k_norm_bound}
\|\epsilon(k)\|_2\leq \|\epsilon(k)\|_1\leq \sum_{i=1}^n(U_2+\epsilon(k)')\leq \sum_{i=1}^n\frac{2\eta\sqrt{n}|\ov{S}_i|}{ m} \left\| u(k) - y \right\|_2.
\end{align}
Notice that
\begin{align*}
\sum_{i=1}^n |\ov{S}_i|=\sum_{r=1}^m \sum_{i=1}^n{\bf 1}_{r\in \ov{S}_i}=\sum_{i=1}^n(\sum_{r=1}^m {\bf 1}_{r\in \ov{S}_i}).
\end{align*}
Hence by Eq. \eqref{eq:Si_size_bound},
with probability at least $1-n\exp(-mR\kappa^{-1})$,
\begin{align*}
\sum_{i=1}^n |\ov{S}_i|\leq 4mnR\kappa^{-1}.
\end{align*}
Plugging the choice of $R=\frac{ 4 \sqrt{n} \| y - u (0) \|_2 }{ \sqrt{m} \lambda }$ and $\|y-u(0)\|_2=O\left(\sqrt{n\log(m/\delta)\log^2(n/\delta)}\right)$,
we have
\begin{align}\label{eq:epsk_norm}
\|\epsilon(k)\|_2 = O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big) \cdot \left\| u(k) - y \right\|_2.
\end{align}

Next we relate $H(k)$ with $H^{\cts}$.
We can rewrite Eq. \eqref{eq:uk_diff} as
\begin{align}\label{eq:uk_diff_cts}
u(k+1)-u(k)=-\eta H^{\cts}(u(k)-y)+\xi(k),
\end{align}
where 
\begin{align*}
\xi(k)=\eta(H^{\cts}-H(k))(u(k)-y)+\epsilon(k).
\end{align*}
Notice that
\begin{align}\label{eq:cts_Hk_diff}
\|H^{\cts}-H(k)\|\leq & ~ \|H^{\cts}-H(k)\|_F\notag\\
\leq & ~ \|H^{\cts}-H^{\dis}\|_F+\|H^{\dis}-H(k)\|_F\notag\\
= & ~ O\left(n\Big(\delta+\frac{ n\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m}  }\Big)\right)+O(n\sqrt{\log(n/\delta)/m})\notag\\
= & ~O\left(\frac{ n^2\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m}  }\right)
\end{align}
where the second step follows from Lemma \ref{lem:HZ_norm_bound} and Lemma \ref{lem:3.1_para}.
Hence we can bound $\xi(k)$ as
\begin{align}\label{eq:xi_bound}
\|\xi(k)\|_2\leq & ~\eta\|(H^{\cts}-H(k))(u(k)-y)\|_2+\|\epsilon(k)\|_2\notag\\
= & ~ O \Big( \frac{ \eta n^2\sqrt{\log(m/\delta)\log^2(n/\delta)}} { \kappa\lambda\sqrt{m} } \Big)\cdot \|u(k)-y\|_2 \notag\\
& ~ + O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big) \cdot \left\| u(k) - y \right\|_2\notag\\
= & ~ O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big)\cdot \left\| u(k) - y \right\|_2,
\end{align}
where the second step follows from Eq. \eqref{eq:epsk_norm} and Eq. \eqref{eq:cts_Hk_diff}.
%\Zhao{The above brackets are not matching before, please check carefully... }

Therefore we have
\begin{align}\label{eq:uk_y}
u(k)-y= & ~u(k)-u(k-1)+u(k-1)-y\notag \\
= & ~-\eta H^{\cts}(u(k-1)-y)+\xi(k-1)+u(k-1)-y\notag\\
= & ~ (I-\eta H^{\cts})(u(k-1)-y)+\xi(k-1)\notag\\
= & ~(I-\eta H^{\cts})^k(u(0)-y)+\sum_{t=0}^{k-1}(I-\eta H^{\cts})^t\xi(k-1-t)\notag\\
= & ~(I-\eta H^{\cts})^ku(0)-(I-\eta H^{\cts})^ky+\sum_{t=0}^{k-1}(I-\eta H^{\cts})^t\xi(k-1-t).
\end{align}
where the second step follows from Eq. \eqref{eq:uk_diff_cts}.
We bound terms on RHS respectively.

Recall that $H^{\cts}=\sum_{i=1}^n \lambda_i v_i v_i^\top$.
Hence $v_1,\cdots,v_n$ are also the eigenvectors of $(I-\eta H^{\cts})^k$ with corresponding eigenvalues $(1-\eta\lambda_1)^k,\cdots,(1-\eta\lambda_n)^k$.
With the choice of $\eta=O(\lambda/n^2)$,
we have 
\begin{align}\label{eq:I-cts_spectrum}
\|(I-\eta H^{\cts})^k\|\leq (1-\eta\lambda)^k.
\end{align}
Therefore
\begin{align}\label{eq:y_bound}
\|-(I-\eta H^{\cts})^ky\|_2^2=\sum_{i=1}^n (1-\eta\lambda_i)^{2k}\langle v_i,y\rangle^2.
\end{align}

We then bound the term $(I-\eta H^{\cts})^ku(0)$.
In the proof of Claim \ref{cla:yu0},
we implicitly prove that with probability at least $1-\delta$,
for all $i\in[n]$,
\begin{align*}
|u_i(0)|\leq \kappa \cdot \sqrt{2\log ( 2mn / \delta) }\cdot \log ( 4n / \delta ).
\end{align*}
And this implies
\begin{align*}
\|u(0)\|_2^2 \leq n\kappa^2 \cdot 2\log ( 2mn / \delta) \cdot \log^2 ( 4n / \delta ).
\end{align*}
Therefore
\begin{align}\label{eq:u0_bound}
\|(I-\eta H^{\cts})^ku(0)\|_2
\leq & ~ \|(I-\eta H^{\cts})^k\|\cdot \|u(0)\|_2 \notag \\
\leq & ~ (1-\eta\lambda)^k \cdot \sqrt{n\kappa^2 }\cdot \sqrt{2\log ( 2mn / \delta) }\cdot \log ( 4n / \delta ).
\end{align}
where the second step follows from Eq. \eqref{eq:I-cts_spectrum}.

Finally, we have
\begin{align}\label{eq:sum_xi_bound}
&~\|\sum_{t=0}^{k-1}(I-\eta H^{\cts})^t\xi(k-1-t)\|_2\notag\\
\leq & ~ \sum_{t=0}^{k-1}\|(I-\eta H^{\cts})^t\| \cdot \|\xi(k-1-t)\|_2\notag\\
\leq & ~ \sum_{t=0}^{k-1}(1-\eta \lambda)^t \cdot O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big) \cdot \left\| u(k-1-t) - y \right\|_2\notag\\
\leq & ~ \sum_{t=0}^{k-1}(1-\eta \lambda)^t \cdot O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big) \cdot (1-\eta\lambda/2)^{(k-1-t)/2}\cdot \|u(0)-y\|_2 \notag\\
\leq & ~ \sum_{t=0}^{k-1}(1-\eta \lambda)^t \cdot O \Big( \frac{\eta n^{5/2}\sqrt{\log(m/\delta)\log^2(n/\delta)}}{\lambda \kappa \sqrt{m}} \Big) \cdot (1-\eta\lambda/4)^{k-1-t}\cdot \sqrt{n\log(m/\delta)\log^2(n/\delta)}\notag\\
\leq & ~ \sum_{t=0}^{k-1}(1-\eta\lambda/4)^{k-1}\cdot O \Big(\frac{\eta n^{3}\log(m/\delta)\log^2(n/\delta)}{\lambda \kappa \sqrt{m}} \Big) \notag\\
= & ~  O \Big(\frac{n^{3}\log(m/\delta)\log^2(n/\delta)}{\lambda^2 \kappa \sqrt{m}}\Big)
\end{align}
where the second step follows from Eq. \eqref{eq:I-cts_spectrum} and Eq. \eqref{eq:xi_bound},
the third step follows from Theorem \ref{thm:quartic},
the fourth step follows from Claim \ref{cla:yu0} and the inequality $(1-x)^{1/2}\leq 1-x/2$,
and the last step follows from $\max_{k\geq 0} k(1-\eta \lambda/4)^{k-1}=O(1/(\eta\lambda))$.


Combining Eq. \eqref{eq:u0_bound}, \eqref{eq:y_bound} and \eqref{eq:sum_xi_bound},
we have
\begin{align*}
\|u(k)-y\|_2= & ~\Big( \sum_{i=1}^n (1-\eta\lambda_i)^{2k}\langle v_i,y\rangle^2 \Big)^{1/2} \\
& ~ \pm O \Big(\sqrt{n\kappa^2 }\cdot \sqrt{2\log ( 2mn / \delta) }\cdot \log ( 4n / \delta )+\frac{n^{3}\log(m/\delta)\log^2(n/\delta)}{\lambda^2 \kappa \sqrt{m}} \Big)^{1/2}\\
= & ~ \left( \sum_{i=1}^n (1-\eta\lambda_i)^{2k}\langle v_i,y\rangle^2 \right)^{1/2} \\
& ~ \pm O\left(\epsilon\right).
\end{align*}
which completes the proof of Theorem \ref{thm:generalization_main}.
\end{proof}

\begin{remark}
The conclusiion in Theorem \ref{thm:generalization_main} can be further strengthened under stronger assumptions on the training data. For example, if part 2 in Assumption \ref{ass:data_dependent_assumption} holds,
notice that
\begin{align*}
\left\|\sum_{j=1}^n ( u_j(k) - y_j ) a_r x_j {\bf 1}_{ w_r(k)^\top x_j \geq 0 }\right\|_2^2
= & ~\sum_{j_1=1}^n \sum_{j_2=1}^n ( u_{j_1}(k) - y_{j_1} )( u_{j_2}(k) - y_{j_2} )x_{j_1}^\top x_{j_2} {\bf 1}_{ w_r(k)^\top x_{j_1} \geq 0,w_r(k)^\top x_{j_2} \geq 0 }\\
= & ~(u(k)-y)^\top H(k)(u(k)-y).
\end{align*}
By part 2 in Assumption \ref{ass:data_dependent_assumption},
we have $\|H(k)\|\leq \alpha$,
therefore
\begin{align*}
\left\|\sum_{j=1}^n ( u_j(k) - y_j ) a_r x_j {\bf 1}_{ w_r(k)^\top x_j \geq 0 }\right\|_2\leq \sqrt{\alpha}\cdot \|u(k)-y\|_2,
\end{align*}
so we can replace Eq. \eqref{eq:eps_k_norm_bound} with
\begin{align*}
\|\epsilon(k)\|_2\leq \sum_{i=1}^n\frac{2\eta \sqrt{\alpha}|\ov{S}_i|}{ m} \left\| u(k) - y \right\|_2.
\end{align*}
Also,
by Theorem \ref{thm:cubic},
we can set $R$ to be $O(\frac{ \sqrt{\alpha} \| y - u (0) \|_2 }{ \sqrt{m} \lambda })$.
Putting everything together,
we have the following Theorem.
\begin{theorem}\label{thm:generalization_main_assumption_2}
Assume Part 1 and 2 of Assumption~\ref{ass:data_dependent_assumption}. 
Recall that $\lambda=\lambda_{\min}(H^{\cts})>0$.
Write the eigen-decomposition of $H^{\cts}$ as $H^{\cts}=\sum_{i=1}^n \lambda_i v_i v_i^\top$ where $v_i\in \mathbb{R}^n$ are the eigenvectors,
and $\lambda_i>0$ are the corresponding eigenvalues.
Let 
\begin{align*}
\kappa = & ~ O( \epsilon / ( \sqrt{2n\log ( 2mn / \delta) }\cdot \log ( 4n / \delta ) ) ) \\
m = & ~ \Omega( \lambda^{-4}\kappa^{-2} n^4\alpha^2 \log (n/\delta) ),
\end{align*}
we i.i.d. initialize $w_r \in {\N}(0,\kappa^2I)$, $a_r$ sampled from $\{-1,+1\}$ uniformly at random for $r\in [m]$, and we set the step size $\eta = O( \lambda / n^2 )$,  then with probability at least $1-\delta$ over the random initialization we have for $k = 0,1,2,\cdots$
\begin{align}
\| u (k) - y \|_2 = \left( \sum_{i=1}^n(1-\eta\lambda_i)^{2k}(v_i^\top y)^2 \right)^{1/2} \pm \epsilon.
\end{align}
\end{theorem}
\end{remark}
